ScopeFlow: Dynamic Scene Scoping for Optical Flow

We propose to modify the common training protocols of optical flow, leading to sizable accuracy improvements without adding to the computational complexity of the training process. The improvement is based on observing the bias in sampling challenging data that exists in the current training protocol, and improving the sampling process. In addition, we find that both regularization and augmentation should decrease during the training protocol. Using an existing low parameters architecture, the method is ranked first on the MPI Sintel benchmark among all other methods, improving the best two frames method accuracy by more than 10%. The method also surpasses all similar architecture variants by more than 12% and 19.7% on the KITTI benchmarks, achieving the lowest Average End-Point Error on KITTI2012 among two-frame methods, without using extra datasets.

==> old_text.tex <==
%%%%%%%%% TITLE
\title{ScopeFlow: Dynamic Scene Scoping for Optical Flow}

\author{Aviram Bar-Haim$^1$ and Lior Wolf$^{1,2}$ \\
$^{1}$Tel Aviv University\\
$^{2}$Facebook AI Research\\
% {\tt\small aviramb@mail.tau.ac.il, wolf@cs.tau.ac.il}
% For a paper whose authors are all at the same institution,
% omit the following lines up until the closing ``}''.
% Additional authors and addresses can be added with ``\and'',
% just like the second author.
% To save space, use either the email address or home page, not both
% \and
% Second Author\\
% Institution2\\
% First line of institution2 address\\
% {\tt\small secondauthor@i2.org}
}

\maketitle
%\thispagestyle{empty}

%% ABSTRACT
\begin{abstract}
We propose to modify the common training protocols of optical flow, leading to sizable accuracy improvements without adding to the computational complexity of the training process. The improvement is based on observing the bias in sampling challenging data that exists in the current training protocol, and improving the sampling process. In addition, we find that both regularization and augmentation should decrease during the training protocol.


Using a low parameters off-the-shelf model, the method is ranked first on the MPI Sintel benchmark among all other methods, improving the best two frames method accuracy by more than 10\%. The method also surpasses all similar architecture variants by more than 12\% and 
{19.7\% }on the KITTI benchmarks, achieving the lowest Average End-Point Error on KITTI2012 among two-frame methods, without using extra datasets.
\end{abstract}

%% Introduction
\section{Introduction}

The field of optical flow estimation has benefited from the availability of acceptable benchmarks. In the last few years, the architectures of choice have stabilized, and a greater emphasis has been {\color{black}placed} on the training protocol.

A conventional training protocol now consists of two stages: (i) pretraining on larger and simpler data and (ii) finetuning on more complex datasets. In both stages, a training step includes the following: (i) sampling batch frames and flow maps, (ii) applying photometric augmentations to the frames, (iii) applying affine (global and relative) transformations to the frames and flow maps, (iv) cropping a fixed size random crop from both input and flow maps, (v) feeding the cropped frames into a CNN~\cite{LeCun:1989:BAH:1351079.1351090} architecture, and (vi) backpropagating the loss of the flow estimation. 

While photometric augmentations include variations of the input image values, affine transformations are used to augment the variety of input flow fields. Due to the limited motion patterns represented by today's optical flow datasets, these regularization techniques are required for the data driven training. We chose the word \textit{scoping}, to define the process of affine transformation followed by cropping, as this process sets the scope of the input frames.

%% Figure - Scatter EPE
\begin{figure}[t]
\begin{center}
    \includegraphics[width=0.99\linewidth]{figures/scatter_mepe.jpg}
    \caption{\textbf{Model size and accuracy trade-off.} Average-end-point-error of the leading methods on the MPI Sintel benchmark vs. the number of trainable parameters. PWC-Net based models are marked in blue. Our model is in the bottom left corner, achieving the best performance with low number of parameters during training.
    $^1$Methods that use more than two frames. $^2$SelFlow uses half of the parameters in test time. $^3$Trained with additional datasets.}
\end{center}
\label{fig:parameters_to_epe}
\end{figure}

To improve optical flow training, we ask the following questions: {Q1.} How do fixed size crops affect this training? {Q2.} What defines a good set of scopes for optical flow? {Q3.} Should regularization be relaxed after pretraining?

Our experiments employ the smallest PWC-Net~\cite{Sun2018PWC-Net} variant of Hur \& Roth~\cite{Hur2019CVPR}, with only 6.3M trainable parameters, in order to support low memory, real time processing. We demonstrate that by answering these questions and contributing to the training procedure, {\color{black}it is possible to train} a dual frame, monocular and small sized model to outperform all other models on the MPI Sintel benchmark. The trained model improves the accuracy of the baseline model, which uses the same architecture, by 12\%. See Fig.~\ref{fig:parameters_to_epe} for a comparison to other networks.

Moreover, despite using the smallest PWC-Net variant, our model outperformed all other PWC-Net variants on both KITTI 2012 and KITTI 2015 benchmarks, improving the baseline model results by 12.2\% and 19.7\%
on the public test set, and demonstrating once more the power of using the improved training protocol. 

Lastly, albeit no public benchmark is available for occlusion estimation, we compared our occlusion results to other published results on the full Sintel dataset, demonstrating more than 5\% improvement of the best published F1 score. 

Our main contributions are:
%\begin{enumerate}
(i) showing, for the first time, as far as we can ascertain, that CNN training for optical flow and occlusion estimation can benefit from cropping randomly sized scene scopes, (ii) exposing the powerful effect of regularization and data augmentation on CNN training for optical flow and (iii) presenting an updated generally applicable training scheme and testing it across benchmarks, on the widely used PWC-Net network architecture.
%\end{enumerate}

Our code is attached as supplementary and our models will be openly shared, in order to encourage follow-up work, to support reproducibility, and to provide an improved performance to off the shelf real-time models.
%------------------------------------------------------------

%% Related work
\section{Related work}
\label{related_works}
% \noindent \textbf{Optical flow foundations.}
% Since the seminal works of Horn \& Schunck~\cite{10.1117/12.965761}, Lucas \& Kanade~\cite{Lucas:1981:IIR:1623264.1623280}, the field of optical flow estimation have seen much progress. These energy minimization formulations conducted the foundations of common assumptions, such as spatial smoothness and brightness constancy, which drive architectures until this decade. These assumptions are the reason for many difficulties in the field until today, such as large displacement or small object motion estimation, and handling of occluded areas~\cite{Brox11,Bruhn2005,5962,ISKB18,Alvarez2007,Sun2014}. While some works formulated the problem with probability measures~\cite{139707,yin2019hd3}, many advances evolved from matching sparse correspondences~\cite{bailer2015iccvflowfields,Hu2016CVPR,7298607} and interpolating them into dense flow fields~\cite{Revaud2015CVPR,Hu2017CVPR}.

%\noindent \textbf{Deep CNNs for optical flow.}
%In the beginning of the deep era
The deep learning revolution in optical flow started with deep descriptors~\cite{6751282,Gadot_2016_CVPR,bailer_patch_match} and densification methods~\cite{Zweig_2017_CVPR}. Dosovitskiy \etal~\cite{7410673} presented FlowNet, the first deep end-to-end network for optical flow dense matching, later improved by Ilg~\etal~\cite{IMSKDB17}, incorporating classic approaches, like residual image warping. Ranjan \& Black~\cite{spynet2017} showed that deep model size can be much smaller with a coarse to fine pyramidal structure. 
Hui \etal~\cite{hui18liteflownet,hui19liteflownet2} suggested a lighter version for FlowNet, adding features matching, pyramidal processing and features driven local convolution. Xu \etal~\cite{xu_2017_dcflow} adapted semi-global matching~\cite{4359315} to directly process a reshaped 4D cost volume %\footnote{$Cost_{I_{1},I_{2}} \in \mathbb{R}^{HW\times{|V|}^2}$ where $V$ is the set of possible velocities and $[H,W]$ is the spatial input images size.} 
of features learned by CNN, inspired by common practices in stereo matching. Yang \& Ramanan~\cite{yang2019vcn} suggested a method for directly learning to process the 4D cost volume, with a separable 4D convolution. Sun~\etal~\cite{Sun2018PWC-Net} proposed PWC-Net, which includes pyramidal processing of warped features, and a direct processing of a partial layer-wise cost volume, demonstrated strong performance on optical flow benchmarks. Many extensions were suggested to the PWC-Net architecture, among them multi-frame processing, occlusion estimation, iterative warping and weight sharing~\cite{ren2018fusion,Neoral2018ACCV,Liu:2019:SelFlow,Hur2019CVPR}. %as explained in Sec.~\ref{related_works:pwc}.

\noindent \textbf{Pretraining optical flow models\quad}
%The role of pre-training as a regularizer was studied in the general domain~\cite{pmlr-v9-erhan10a}, and shown to restrict a follow-up training parameters space. Mahajan \etal~\cite{Mahajan_2018_ECCV} showed that labelspace fit to a fine-tune dataset is more important than the pre-training dataset magnitude.
Today's leading optical flow learning protocols, include  pretraining on large scale data. The common practice is to pretrain on the FlyingChairs~\cite{7410673} and then on FlyingThings3D~\cite{things3d} (FChairs and FThings). As shown by recent works~\cite{Mayer_2018,IMSKDB17}, the multistage pretraining ordering is critical. The FChairs dataset includes 21,818 pairs of frames, generated by CAD models~\cite{seeing_3d_chairs}, with flicker images background. FThings is a natural extension of the FChairs dataset, having 22,872  larger 3D scenes with more complex motion patterns. Hur \& Roth~\cite{Hur2019CVPR} created a version of FChairs with ground truth occlusions, called FlyingChairsOcc (denoted FChairsOcc), to allow supervised pretraining on occlusion labels.

\noindent \textbf{Datasets and benchmarks\quad} 
%Unlike other fields in computer vision, realistic optical flow annotated data is very difficult to obtain~\cite{4587845,Wulff:ECCVws:2012}. The rise of small flow datasets, such as the famous Yosemite~\cite{Barron1994}, Middlburry~\cite{Baker2011} and others, demonstrated the power of annotated data to the field of optical flow. 
The establishment of large complex benchmarks, such as MPI Sintel~\cite{Butler:ECCV:2012}, and KITTI~\cite{Geiger2012CVPR,Menze2015CVPR}, boosted the evolution of optical flow models. The MPI Sintel dataset was created from the Sintel movie, composed of 25, relatively long, annotated scenes, with 1064 training frames in total. The final pass category of Sintel is a challenging one, having many realistic effects to mimic natural scenes. The KITTI2012 dataset comprises 194 training pairs with annotated flow maps, while KITTI2015 has 200 dynamic color training pairs. Furthermore, some methods are using more datasets during the finetune process, such as HD1K~\cite{kondermann2016hci}, Driving and Monkaa~\cite{things3d}.

%\noindent \textbf{Challenging motion categories.} 
%Flow map pixels can be categorized by multiple criteria, for instance: large and small displacements, occluded and non occluded pixels, and distance from the closest object or image boundary. Naturally, different methods excel in specific categories while poorly solving other motion profiles. 
\noindent \textbf{Motion categories\quad}
MPI Sintel provides a stratified view of the error magnitude of challenging motion patterns. The ratio of the best mean error for the small motion category (slower than 10 pixels per frame) to the large motion category (faster than 40 pixels per frame) is approximately x44. 
% best mean error for the category of small motion (with velocities lower than 10 pixels per frame) is 0.582 pixels, the best mean error for the category of large motion (with velocities larger than 40 pixels per frame) is 25.5 pixels (x44). 
In Sec.~\ref{method:scene_scoping}, we present one possible theoretical explanation for the poor performance of state of the art methods in large motions, and suggest an approach to improve the accuracy of this pixels category.

Another example is the category of unmatched pixels. This category includes pixels belonging to regions that are visible only in one of two adjacent frames (occluded pixels). As expected, these pixels share much higher end-point-error than match-able pixels: the ratio of the best match-able EPE to the best non match-able is approximately 9.5.

Different deep learning approaches were suggested to tackle the problems of fast objects and occlusion estimation. Among the different solutions suggested were: occlusion based loss~\cite{occlusion_sep} and model~\cite{Liu:2019:DDFlow,Liu:2019:SelFlow} separation, and multi-frame support for long-range, potentially occluded, spatio-temporal matches~\cite{ren2018fusion,Neoral2018ACCV}. We suggest a new approach for applying multiple strategies online. Our findings imply that the training can be improved by applying scene scope variations, while taking into account the probability of sampling valid examples from different flow categories.


\noindent \textbf{Training procedure and data augmentation\quad}
Fleet \& Weiss~\cite{Fleet2006OpticalFE} showed the importance of photometric variations, boundary detection and scale invariance to the success of optical flow methods. In recent years, as the evolution of optical flow models started to saturate, training variation studies became more popular~\cite{Liu:2019:SelFlow}.  Sun~\etal~\cite{Sun2018:Model:Training:Flow} used training updates to improve the accuracy of the initial PWC-Net model by more than 10\%, showing they could improve the reported accuracy of FlowNetC (a sub network of FlowNet) by more than 50\%, surpassing FlowNet2~\cite{hui19liteflownet2} performance, with their updated training protocol. %They concluded that for a fair data driven models comparison, a training process has to be fixed. 
Mayer \etal~\cite{Mayer_2018} suggests that no single best general-purpose training protocol exists for optical flow, and different datasets require different care. These conclusions are in line with our findings on the importance of proper training.

%\noindent \textbf{Dealing with occlusions} 
%The need for multiple targets in optical flow estimation, to overcome the traditional limitations, was studied in different contexts~\cite{Mayer_2018,Schuster2016OpticalFR,ISKB18}. Brox \& Malik~\cite{Brox11} suggested that classic descriptors, such as SIFT~\cite{Lowe2004} and HOG~\cite{1467360}, suffer from bad localization in the context of dense matching, and proposed to combine them into the variational framework, to handle both small and large objects. Xiao \etal~\cite{bilateral_occlusion} added an occlusion term to the flow energy functional. In the deep era, 

% \noindent \textbf{Random cropping}
% {\color{red}REMOVE? In the beginning of the deep learning era,} Krizhevsky \etal~\cite{alexnet} showed that image resize and cropping augmentations only helped them to win the ImageNet challenge~\cite{imagenet_cvpr09}. Later, Szegedy~\etal~\cite{7780677_Szegedy} showed that models with low parameters could produce great classification results when considering the receptive field and cropping strategy. In the optical flow domain, cropping was used to augment the flow~\cite{Sun2018PWC-Net}, and occlusions~\cite{Liu:2019:DDFlow}, using a randomly located fixed size crops. For example, the common practice in PWC-Net based models, when training a model on the MPI-Sintel dataset, is to crop patches of size $[384,768]$, which are 88\% and 75\% of the full image height and width of $[436,1024]$. Another example is the KITTI dataset, where a fixed crop size of $[320,896]$ is used, which are 86.4\% and 87.5\% out of the full image size $[370,1240]$. 

% While we found that random cropping and geometric transformations are indeed an important source of regularization, we suggest they have another important role, of controlling the scope of the scene. The scene scope defines the visibility of different motion patterns, such as velocity categories and occluded pixels, which are a primary source of information in a data driven learning process.

%% Method - PWC-Net
\subsection{PWC-Net architectures}
\label{related_works:pwc}
PWC-Net~\cite{Sun2018PWC-Net} is the most popular architecture for optical flow estimation to date, and many variants for this architecture were suggested~\cite{ren2018fusion,Melekhov+Tiulpin+Sattler+Pollefeys+Rahtu+Kannala:2018,Hur2019CVPR,Liu:2019:SelFlow,Neoral2018ACCV}. PWC-Net architecture was built over traditional design patterns for estimating optical flow, given two temporally consecutive frames, such as: pyramidal coarse-to-fine estimation, cost volume processing, iterative layerwise feature warping and others. 
\noindent \textbf{Features warping\quad} In PWC-Net, a CNN encoder creates feature maps for the different network layers (scales). The features of the second image are backward warped, using the upsampled flow of the previous layer processing, for every layer $l$, except the last layer $l_{Top}$, by:
% In PWC-Net forward pass, a CNN feature encoder encodes the two input images, and creates feature maps for the different network layers (scales). The features of the second image are backward warped, using the upsampled flow of the previous (coarser) layer processing, for all layers $l~~ s.t.~~ {l<l_{Top}}$ by:
\begin{equation}
    \label{warping}
    c_{w}^{l}(x) = c_{2}^{l}(x + up_{\times2}(f^{l+1}(x))
\end{equation}
where x is the pixel location, $c_{w}^{l}(x)$ is the backward warped feature map of the second image, $f^{l+1}(x)$ is the output flow of the coarser layer, and $up_{\times2}$ is the $\times2$ up-sampling module, followed by a bi-linear interpolation.

\noindent \textbf{Cost volume decoding\quad} A correlation operation applied on the first and backward warped second image features, in order to construct a cost volume:
\begin{equation}
\label{eq:correlation}
    cost^{l}(x_{1}, x_{2}) = \frac{1}{N}(c_{1}^{l}(x_{1}))^{T}c_{w}^{l}(x_{2})
\end{equation}
{where $c_{n}^{l}(x)\in \mathbb{R}^N$ is a feature vector of image n.}

The cost volume is then processed by a CNN decoder, in order to estimate the optical flow directly. In some variants of PWC-Net~\cite{Neoral2018ACCV,Hur2019CVPR} there
is an extra decoder with similar architecture for occlusion estimation.

% \noindent \textbf{Cost volume decoders.} The cost volume, which holds a more discriminative representation of feature matches of pixels, being processed by a CNN decoder, in order to estimate the optical flow directly. In some variants of PWC-Net~\cite{Neoral2018ACCV,Hur2019CVPR} there is another decoder network, with the same architecture of the optical flow decoder, that estimates occlusion from the cost volume directly.


\noindent \textbf{Iterative residual processing\quad} 
Our experiments employ the Iterative Residual Refinement proposed by Hur \& Roth~\cite{Hur2019CVPR}.
% , which uses shared weights for the different coarse to fine layers. 
The reasons we chose to test our changes for the PWC-Net architecture on the IRR variant are: 
(i) IRR has the lowest number of trainable parameters among all PWC-Net variants, making a state of the art result obtained with proper training more significant, (ii) it uses shared weights that could be challenged with scope and scale changes, and if successful, it would demonstrate the power of a rich, scope invariant feature representations, (iii) this variant is using only two frames - demonstrating the power of dynamic scoping without long temporal connections, (iv) the occlusion map allows the direct evaluation of our training procedure on occlusion estimation, and (v) any success with this variant directly translates to real-time relatively low complexity optical flow estimation.

% (i) IRR has the lowest number of trainable parameters among all PWC-Net variants, making a state of the art results obtained with proper training more significant. (ii) The weights sharing constraint could be challenged with scope and scale changes, and if successful, it would demonstrate the power of a rich, scope invariant feature representations. (iii) This variant is using only two frames - demonstrating the power of dynamic scoping without long temporal connections. (iv) The occlusions map allows the direct evaluation of our training procedure on occlusion estimation. (v) Any success with this variant directly translates to real-time relatively low complexity optical flow estimation.

% {\color{red}
% DELETE IF NEEDED

% The flow in each IRR-PWC iteration is calculated by:
% \begin{equation}
% f_{fw}^{i} = D(c_{1}^{i}, cost^{i}_{1,w}, \hat{f}_{fw}^{i-1}) + \hat{f}_{fw}^{i-1}
% \end{equation}
% Where $D$ is the optical flow shared decoder, $i$ is the iteration number equivalent to the $l_{Top}-i$ layer in PWC-Net, $c_{1}^{i}$ are the features of the first image in iteration $i$, $cost^{i}_{1,w}$ is calculated in \ref{eq:correlation}, and $\hat{f}_{fw}^{i-1}$ is the $\times2$ upsampled flow from the previous iteration.
% }

%% Method
\section{Scene scoping analysis}

%% 1D random cropping scheme
\begin{figure}[t]
    \centering
    \includegraphics[width=0.85\linewidth]{figures/cropping_scheme_v4.png}
    \caption{{\bf Illustration of Lemma 1}. The probability for a pixel to be sampled within a valid random crop location, depends on the image width $W$, the crop width $w$ and the distance to the closest border $\Delta x$. For both samples $W=8$. Top: $w=3$ ($w \in Crops_{small}$). Bottom: $w=5$ ($w \in Crops_{large}$). Each pixel is labeled with $\Delta x$.}
\label{fig:1dprob}
\end{figure}

%\subsection{Scene scoping}
\label{method:scene_scoping}
Due to the limited number of labeled examples available for optical flow supervised learning, most of the leading methods, in both supervised and unsupervised learning, are using cropping of a \textbf{fixed sized} randomly located patches. We are interested in understanding the chances of a pixel to be sampled, within a randomly located fixed size crop, as a function of its location in the image.

\noindent \textbf{1D image random cropping statistics\quad}
Consider a 1D image with a width $W$, a crop size $w$ and a pixel location $x$.
Let $\Delta x$ denote the distance of the pixel from the closest border, and $\Delta w$ denote the difference between the image width $W$ and the crop size $w$. Let $Crops_{large}$ be the set of crop sizes with $w$ larger than half of the width, $\frac{W}{2} < w\leq W$. Let $Crops_{small}$ be the complement set of crop sizes smaller or equal to half of the width, $0 < w\leq \frac{W}{2}$. Two instances of this setup are depicted in Fig.~\ref{fig:1dprob}.


Using the notations above, the pixels are separated into three different categories, described in the following lemma. 
\begin{lemma}
For an image size $W$ and a randomly chosen crop of size $0<w \leq W$ the probability of a pixel, with coordinate $x$ and distance to the closest border $\Delta x$ to be sampled, is as follows:
\begin{equation}
    P(x| W,w) =
    \begin{cases*}
      1 & if $\Delta w<\Delta x$  \\ %\label{greenprob}
      \frac{w}{\Delta w + 1} & if $ w\leq\Delta x$ \\ %\label{orangeprob}
      \frac{\Delta x}{\Delta w + 1} & otherwise %\label{redprob}
    \end{cases*}
\label{casesprob}
\end{equation}
where $\Delta w + 1$ is the number of valid crops. 
\end{lemma}
\begin{proof}
For illustration purposes, the three cases are color coded, respectively, as green, orange, and red, in Fig.\ref{fig:1dprob}. We handle each case separately.
%Let us define a valid crop placement as a placement with $w$ pixels inside the image borders.
(i) \textbf{Green}: Every valid placement must leave out up to $\Delta w$ pixels from the left or the right. Since $\Delta x$ is larger than $\Delta w$, the pixel $x$ must be covered. (ii) \textbf{Orange}: In this case, there are $w$ possible locations for pixel $x$ within the patch, all of which are achievable, since $\Delta x$ is large enough. Therefore, $w$ patch locations out of all possible patches contain pixel $x$. (iii) \textbf{Red}: In this case, the patch can start at any displacement from the edge that is nearer to $x$, that is not larger than $\Delta x$, and still cover pixel $x$. Therefore, there are exactly $\Delta x$ locations out of the $\Delta w + 1$ possible locations.
\end{proof}

%% Figure - Random cropping effect
\begin{figure*}
\begin{center}
  \includegraphics[width=0.98\linewidth]{figures/figure_3.jpg}\vspace{-.4cm}
% \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
\end{center}
   \caption{\textbf{Sampling bias caused by fixed size random crops.} {\color{black}(a),(b),(c): Pixel sampling probability maps for a fixed sized crop, with a ratios of 50\%, 70\% and 90\% respectively, for each axis. The probability to sample a marginal pixels shrinks drastically with the crop size. (d),(e): areas with strong prevalence for motion categories. High velocities tend to start from lower corners, while small ones tend to occur in the middle and upper part of the scene. (f),(g): graphs of the changing ratio of sampling probabilities between fast ($>40$) and slow ($<10$) pixels, for different crop and image axes ratios. clearly, fast pixels benefit more when increasing the crop size than slow pixels.}}
\label{fig:pixel-prob-per-crop-size}
\end{figure*}

\noindent \textbf{2D image random cropping statistics\quad}
Since the common practice in current state-of-the-art optical flow training protocols is to crop a fixed sized crop, in the range
$\frac{W}{2}<w\leq W$ \((w \in Crops_{large})\),
% $\frac{W}{2}<w<W$ \((w \in Crops_{large})\), 
we will focus in the reminder of this section on the green and red categories, which are the relevant categories for crop sizes with each dimension [h,w] larger than half of the corresponding image dimension (\ie in $Crops_{large}$), and represent a cropping of more than a quarter of the image.

From the symmetry of our 1D random cropping setup, in both $x$ and $y$ axes, we can use Eq.~\ref{casesprob} in order to calculate the probability of sampling pixels in a 2D image of size $[H,W]$, with a randomly located crop of a fixed size $[h,w]$. The probability of sampling a central (green) pixel remains 1, while the probability of sampling a marginal (red) pixel $(x,y)$ in 2D, is given by:
\begin{equation}
\label{eq:2d_margin_prob}
P_{red}(x,y | H,h,W,w) = \frac{\min{(\Delta x, \Delta w)}\min{(\Delta y, \Delta h)}}{(\Delta w + 1)(\Delta h + 1)}
\end{equation}
Where $\Delta h = H-h$, $\Delta w = W-w$ the difference between the image and the crop width and height, and $\Delta x, \Delta y$ represent the distance from the closest border, as before. Eq.~\ref{eq:2d_margin_prob} represents the ratio between the number of crop locations where a (marginal) pixel with $\Delta x, \Delta y$ is sampled to the number of all unique valid crop locations. An illustration of this sampling probability is demonstrated in Fig.~\ref{fig:pixel-prob-per-crop-size} for varying ratios of crop size axes and image axes.

\noindent \textbf{Fixed crop size sampling bias\quad}
As in the 1D cropping setup, given an image of size $[H,W]$ and a crop size $[h,w]$, we can define a central area (equivalent to the green pixels in 1D), which will always be sampled. Respectively, we can define a marginal area (equivalent to the red pixels in 1D), where Eq.~\ref{eq:2d_margin_prob} holds.

Eq.~\ref{casesprob} links this marginal area to the values $\Delta h$ and $\Delta w$.  %{\color{red}REMOVE THE FOLLOWING SENTENCE?}This means that there is a margin with height $\Delta h$ and width $\Delta w$ where Eq.~\ref{eq:2d_margin_prob} holds, and all non-marginal pixels will be sampled in all crops. Moreover, 
Analyzing Eq.~\ref{eq:2d_margin_prob} we can infer the following: (i) in the marginal area, for a fixed crop size $[h,w]$, the probability of being sampled decreases quadratically along the image diagonal, when $\Delta x$ and $\Delta y$ both decrease together, and (ii) in the marginal area, for a fixed pixel, the probability of being sampled decreases quadratically when the crop size decreases (when $\Delta w$ and $\Delta h$ both decrease together).

Therefore, when using a fixed sized crop to augment a dataset with a random localization approach, there will be a dramatic sampling bias towards pixels in the center of the image, preserved by the symmetric range of random affine parameters. For example, with the current common cropping approach for the MPI Sintel data-set, the probability of the upper left corner pixel to be sampled in a crop equals \(\frac{1}{(1024-768 + 1)(436 - 384 + 1)} = 0.000073\%\), while the pixels in the central $[332,512]$ crop will be sampled in any randomized crop location. %This ratio 1:13621 is also the ratio of the largest sampling discrepancy between two pixels.

This sampling bias could have a sizable influence on the training procedure. Fig.~\ref{fig:pixel-prob-per-crop-size} illustrates the distribution of fast pixels in both MPI Sintel and KITTI datasets. Noticeably, pixels of fast moving objects (with speed larger than 40 pixels per frame) are often located at the marginal area, while slower pixels are more centered in the scene. This should not be a surprise, since (i)  lower pixels belong to nearer scene objects and thus have a larger scale and velocity, and (ii) fast moving objects usually cross the image borders.

Moreover, many occluded pixels are also located close to the image borders. Therefore, increasing a crop size could also help to observe a more representative set of occlusions during training. Therefore, we hypothesized that larger crops can also improve the ability to infer occluded pixels motion from the context. 

\subsection{Scene scoping approaches}
\label{method:scoping_approaches}
Fig.~\ref{fig:pixel-prob-per-crop-size} shows the crop size effect on the probability to sample different motion categories. Clearly, the category of fast pixels suffers the most from reduction of the crop sizes. We tested four different strategies for cropping the scene dynamically (per mini batch) during training:
(S1) fixed partial crop size (the common approach), (S2) cropping the largest valid crop size, {\color{black}(S3) randomizing crop size ratios from a pre-defined set with:
    \begin{subequations}
        \begin{equation}
            \label{eq:rcrop_size_fixed}
            R_{fixed} = \{(0.73,0.69),(0.84,0.86),(1,1)\}
        \end{equation}
        \begin{equation}
                \label{eq:rcrop_size_set}
                (r_{h},r_{w})= 
                randchoice(R_{fixed}),
        \end{equation}
    \end{subequations} where $(r_{h},r_{w})$ are one of the three crop ratios, 
    and strategy (S4) is a range-based crop size randomization:
    \begin{equation}
        \label{eq:rcrop_size_range}
        s=randint(round(r_{min} \cdot S), round(r_{max} \cdot S)),
    \end{equation}
    where s is the crop axis size (h or w), S is the full image axis size (H or W), and [$r_{min}$, $r_{max}$] is the range of crop size ratios $\frac{s}{S}$ for sampling.
}

We also employ different affine transformations, and dynamically change the zooming range along the training, to enlarge the set of possible scene scopes, and improve the robustness of features to different scales. In Sec.~\ref{experiments:full_train} we describe the experiments done in order to find an appropriate approach for feeding the network with a diversity of scene scopes and reducing the inherent sampling bias explained in this section, caused by the current cropping mechanisms.

\begin{figure}
    \begin{center}
    \includegraphics[width=0.98\linewidth]{figures/min_crop_range_mepe_v8.jpg}
    \end{center}
    \caption{Accuracy of models trained with different ranges of random crop sizes, on the combined KITTI dataset. The maximal crop size is the full image. Validation AEPEs improve when increasing the minimal crop size ratio ($r_{min}$ in Eq.\ref{eq:rcrop_size_range}) up to 95\% of the full image (on each axis). AEPE for a fixed sized crop based training in red.}
\label{fig:min_crop_comparison}
\end{figure}

%\ifinline {\color{red} MAYBE A FIGURE COMPARING THE DISTRIBUTION OF PATCHES FOR EACH CATEGORY BY SAMPLING 20 FRAMES FROM EACH METHOD?} \fi

In addition to testing the scope modifications based on our analysis, we were also interested in testing different parameters of the training.


\section{Training, regularization and augmentation}
\label{method:training}
%Although the datasets scheduling studied by some works~\cite{Mayer_2018,ISKB18}, the importance of pre-training gains on the fine-tuning stages is not well understood yet. %In section \ref{experiments} we conducted experiments testing different training changes on different datasets in the common training pipeline.
%\noindent \textbf{PWC-Net base model.} 

\noindent \textbf{Learning rate and training schedules\quad}
\label{method:lr_sched}
The common LR schedules, proposed by Ilg~\etal~\cite{IMSKDB17}, used to train deep optical flow networks are $S_{long}$ or $S_{short}$ for the pretraining stage, and $S_{ft}$ for the finetune phases. We used the shorter schedule, suggested by~\cite{Hur2019CVPR}, of using $S_{short}$ for pretrain, half of $S_{short}$ for FThings finetuning, and $S_{ft}$ for Sintel and KITTI datasets. We also examine the effect of retraining and over-training specific stages {\color{black}of the multi-phase training.}

%These are repetitive decaying schedules of the learning rates, starting from $1e^{-4}$, where the LR is divided in pre defined stages. 
% {\color{blue}TODO CHECK IF LR DECAY CHANGES WERE IN OR NOT}
% , in order to reach better minimas, during different stages of the multi-stage training.

\noindent \textbf{Data augmentation\quad}
\label{method:augmentation}
The common practice in the current training protocol employs two types of data augmentation techniques: photo-metric and geometric augmentations. The details of these augmentations did not change much since FlowNet~\cite{7410673}. The photo-metric transformations include input image perturbation, such as color
% (brightness, contrast, saturation, hue) 
and gamma corrections. The geometric augmentations include a global or relative affine transformation, followed by random horizontal and vertical flipping. Due to the spatial symmetric nature of the translation, rotation and flipping parameters, we decided to focus on the effect of zooming changes, followed by our new cropping approaches.


% {\color{blue}, very large number of possible changes, and the length of the training, we focused in this work on the scope affecting augmentations, which are affine transformations and flipping, followed by cropping. TODO: EDIT AFTER REVISITING FLIP/TRANS/ROT EXPERIMENTS.{\color{red} BE SPECIFIIC}}

% {\color{blue}Due to the very large number of possible changes, and the length of the training, we focused in this work on the scope affecting augmentations, which are affine transformations and flipping, followed by cropping. TODO: EDIT AFTER REVISITING FLIP/TRANS/ROT EXPERIMENTS.{\color{red} BE SPECIFIIC}}
% of either both input images and the flow map or only the second image

\noindent \textbf{Regularization\quad}
\label{method:reg}
The common protocol also includes weight decay and adding random Gaussian noise to the augmented image. In our experiments, we tested the effect of eliminating these sources of regularization at different stages of training.
% random noise and weight decay at different stages of training.
%{\color{blue} REMOVED DETAILS SINCE REMOVING NOISE IN FINETUNE ALWAYS GOOD, REMOVING WD IN FINETUNE GOOD FOR SINTEL ONLY.}

\section{Experiments}
\label{experiments}

\input{manytables.tex}

In this section, we describe the experiments and results for our research questions. Specifically, we tested (i) how can we change the current training pipeline in order to improve the final accuracy, and (ii) the effect of feeding the network with different scopes of the input during training, using different cropping approaches and changes to the zooming parameters.

All our experiments on KITTI used both KITTI2012 and KITTI2015, and for Sintel both the clean and final pass, for training and validation sets. We denote the combined datasets of Sintel and KITTI as Sintel combined and KITTI combined.
We also tested the approach, suggested by Sun~\etal~\cite{Sun2018PWC-Net}, to first train on a combined Sintel dataset, followed by another finetune
% training
on the final pass.

% In some experiments, we followed the approach, suggested by Xu \etal~\cite{xu_2017_dcflow}, to first train on a combined Sintel dataset, consisting of both clean and final pass, followed by another training on the final pass.
% All our experiments on KITTI used both KITTI2012 and KITTI2015 for training and validation together. We denote the combined datasets of Sintel (KITTI) as Sintel combined (KITTI combined).

All of our experiments employ the common End Point Error metric for flow evaluation, and F1 for occlusion evaluation. The KITTI experiments also present the outlier percentage ($> 3$ pixels) metric.


%% Experiments
\subsection{Finetuning a pretrained model}
\label{experiments:finetune}

\input{manytables2.tex}

Since the cost of pretraining is approximately $\times 7$ than of the final finetune, we first present experiments done on the finetuning phase, in which we employ models pretrained on FChairs and FThings, published by the authors of IRR-PWC. {\color{black}These experiments are conducted on the Sintel dataset, since it has similar statistics of displacements to the FChairs dataset~\cite{Mayer_2018} used for pretraining}. We tested different
training protocol changes, and found that substantial gains could be achieved using the following changes:
\noindent \textbf{1. Cropping strategies.} 
During the initial finetune, we tested the cropping approaches specified in Sec.~\ref{method:scoping_approaches} on Sintel. The results specified in Tab.~\ref{tab:ablation} show that the range-based crop size randomization approach (Eq.~\ref{eq:rcrop_size_range}) was comparable to taking the maximal valid crop (although much more efficient computationally), and both improved Sintel validation error of models trained with smaller fixed crop sizes.
% approaches {\color{blue}\#1 (fixed partial), \#2 (maximal valid) and \#4 (range based random) from Sec.~\ref{method:scoping_approaches}, for selecting the crop size}

\noindent \textbf{2. Zooming strategies.} 
We found that applying a new random zooming range of $[0.8,1.5]$ alone, which increases the zoom out, and gradually reducing the zoom in to $1.3$, achieved considerable gains for Sintel
% {\color{red}DELETE and KITTI}
in all evaluation parameters, with and without cropping strategy changes. Interestingly, increasing the zoom out range without any change to the crop size provided 50\% of this gain.
% {\color{red}DELETE  for Sintel}
We suggest that this is additional evidence for the existing bias in small crop sizes, as explained in Sec.~\ref{method:scene_scoping}. 

\noindent \textbf{3. Removing artificial regularization.} 
Removing the random noise and weight decay helped us to achieve extra 2\%-3\% of improvement during {\color{black}Sintel finetune,}
% {\color{red}DELETE for both Sintel and KITTI validation, }
demonstrating the benefit of reducing augmentation {\color{black}in advanced stages.}
% {\color{red}DELETE during finetune.}
% However, we found that the removal of random noise alone to provide more than 2\% of the gain during finetune. This might be due to the importance of spatial features in the domain of motion estimation. {\color{red}NO TABLE THOUGH. TRY NOT TO DISCUSS THINGS THAT ARE NOT IN A TABLE. BETTER TO REMOVE}

\subsection{Applying changes to the full training procedure}
\label{experiments:full_train}
We then tested {\color{black}the changes from Sec.~\ref{experiments:finetune}, along with all four cropping approaches described in Sec.~\ref{method:scoping_approaches},}
% these changes, along with the cropping approaches described in Sec.~\ref{method:scoping_approaches},
on the different stages of the common curriculum learning pipeline. Since we wanted to test our training changes and compare our results to other variants of the baseline architecture, we decided not to use any other dataset other than the common pretraining or benchmarking datasets. For FChairs and FThings, all trained models were evaluated on Sintel training images, as an external test set.

\noindent \textbf{FChairs pretraining\quad} For pretraining, we downloaded the newly released version of FChairs~\cite{Hur2019CVPR}, which includes occlusions ground truth annotations. We trained two versions of the IRR-PWC model on FChairsOCC, for 108 epochs on 4 GPUs: (i) C1: removing weight decay and random noise (ii) C2: same as (i) with reduced zoom in. We then evaluated both models and the original model, trained by the authors with weight decay and original zoom in of $1.5$, denoted by C*. Results are depicted in Tab.~\ref{tab:chairs_training}, showing that regularization is important in early stages, since removing either weight decay and random noise, or reducing the zoom-in hurt the performance. 

\noindent \textbf{FThings finetune\quad} We then trained three versions of IRR-PWC on FThings, for 50 epochs: (i) T2: resuming C* training with batch size of 2, with the original crop size of $[384,768]$, (ii) T3: resuming C1 with the maximal crop size, and (iii) T4: resuming T3 without weight decay and random noise.
% We then evaluated all models and the authors model, trained with weight decay and original crop size, denoted by T*. 
We can infer from the results in Tab.~\ref{tab:things_over_train}: (i) increasing the scope during FChairs training leads to better accuracy on the Sintel test set, and (ii) over-training without weight decay and random noise did not improve the results on the external test set (but did on the validation).
% crop size reduced the error on the Sintel test set.

% \noindent \textbf{FlyingThings3D fine-tune.} We then trained 4 versions of IRR-PWC on FThings, for 50 epochs and on 4 GPUs: (i) T1: resuming C* training with batch size of 6, with the original crop size of $[384,768]$, (ii) T2: same as T1 with a batch size of 2 (iii) T3: resuming C1 with the maximal crop size, and (iv) T4: resuming T3 without weight decay and random noise. We then evaluated all models and the original model, trained by the authors with weight decay and original zoom in of $1.5$, denoted by T*. We can infer from the results in Tab.~\ref{tab:things_bs}  and Tab.~\ref{tab:things_over_train}: (i) using a lower batch size leads to a lower validation and external test error, (ii) over-training without weight decay and random noise did not improve the results on the external test set (but did on the validation), and (iii) increasing the crop size reduced the error on the Sintel test set.
%{\color{blue} 
%T3 AND T4 TRAINED WITH BOTH MAX CROP AND ZOOM OUT (0.8,1.5) WHILE T1,T2,T* USED THE DEFAULT IRR ZOOM OF (1,1.5), SHOULD WE MENTION AND ADD TO TABLE OR KEEP FOR SIMPLICITY?}

\noindent \textbf{KITTI finetune\quad} We trained two different versions, both with the same protocol, for 550 epochs on KITTI combined: (i) resuming T2 and (ii) resuming T3. Although T3 got better performance in the evaluation, after finetuning, both results were similar on KITTI validation, as shown in Tab.~\ref{tab:kitti_pre_train_effect}.

\noindent \textbf{Sintel finetune\quad} Two different versions were trained with the same protocol, for 290 epochs on Sintel combined, both from T3: (i) with weight decay and random noise and (ii) without weight decay and random noise. The results, presented in Tab.~\ref{tab:sintel_finetune_reg}, show that reducing regularization in Sintel finetune produced an extra gain.

% We also tested the best order to fine-tune Sintel, and as shown in Tab.~\ref{tab:sintel_finetune_order} and suggested by~\cite{xu_2017_dcflow}, training on Sintel combined and then on final produced the best results on the combined validation set.

% Figure - fast and occluded pixels improvement
\begin{figure*}[t]
%\begin{center}
% \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
\centering
%   \includegraphics[width=0.9\linewidth]{figures/ambush_comparison.png} % OPTION 1
  \includegraphics[width=0.99\textwidth]{figures/sintel_fast.jpg} % OPTION 2

%\end{center}
   \caption{\textbf{Improving estimation for fast moving pixels.} {\color{black}A qualitative comparison with the other two leading methods on the Sintel benchmark. Images were downloaded from MPI Sintel website, evaluated online on a test image, for the category of fast pixels (40+). Left to right: averaged first and second image and flow visualization for each method. $EPE_{40+}$ is the end point error calculated on fast pixels.}}
\label{fig:occ-fast-improve}
\end{figure*}

\noindent \textbf{Dynamic scene scoping\quad}
Since the scoping approaches were already tested on Sintel during the initial finetune, we further tested the four different approaches for dynamic scene scoping, detailed in Sec.~\ref{method:scoping_approaches}, on the combined KITTI dataset. The results are depicted in Tab.~\ref{tab:randcrop}. For KITTI, cropping the maximal valid crop per batch shows noticeable improvement from using a fixed sized crop. However, for KITTI datasets, approach S4 (Eq. \ref{eq:rcrop_size_range}) show much better performance than using the maximal valid crop size. In order to find the optimal range of crop size ratios (Eq.\ref{eq:rcrop_size_range}), we trained different models with different ranges of crop size to image ratios $[r_{min},r_{max}]$. All models used an upper crop size ratio limit $r_{max}$ equal to 1 (\ie the maximal valid crop for the batch), and different lower limit $r_{min}$, ranging from $0.5$ to $1$ and representing random crop sizes with different aspect ratios, which are larger than a quarter of the image.

Fig.~\ref{fig:min_crop_comparison} shows the training and validation accuracy as a function of the lower ratio of the range of randomized crop sizes. Specifically, the best results obtained with $r_{min}$ equals the 0.95, as also demonstrated in Fig.~\ref{fig:min_crop_comparison}. The validation accuracy improves consistently when increasing $r_{min}$ from 0.5 to 0.95 and then starting to deteriorate until $r_{min}$ is reaching the maximal valid crop size. As can be seen, when enlarging the crop size expectation, we also reduce the regularization provided by the larger number of scopes (as analyzed in Eq.\ref{eq:2d_margin_prob}). %This observed to affect the training on KITTI benchmark, where the number of training samples is less than half of Sintel's. 
This observation can be considered as additional evidence of a regularization-accuracy trade-off in the training process. %Moreover, it shows once more the importance of finding the appropriate augmentation protocol for different datasets. 
It also emphasizes the power of Eq.~\ref{eq:rcrop_size_range}, in improving the training outcome, while keeping the regularization provided by partial cropping.

% {\color{red} THIS RANGE SEEMS QUITE SMALL, NO?} {\color{blue} YES BUT IT CAN MAYBE BECAUSE OF THE ADVANTAGES OF LARGER CROP SIZES IN TERMS OF MARGINAL PIXELS BIAS, AS WE SUGGESTED IN \ref{method:scene_scoping}, AS LONG AS THE LARGER AUGMENTATION OF SMALLER CROP SIZES IS NOT NEEDED. FOR EXAMPLE IN SINTEL USING THE MAXIMAL SIZE ONLY LEADS TO COMPARABLE RESULTS TO THE RANDOM APPROACHES (AND SINTEL HAS MORE THAN X2 SAMPLES). SEE FIGURE ~\ref{fig:min_crop_comparison}.}

\noindent \textbf{Re-finetune with dynamic scene scoping\quad}
In order to further understand the effect of this regularization-accuracy trade-off, we re-trained three models with the best random approach $([r_{min},r_{max}] = [0.95,1])$ on the KITTI combined set, using the same finetuning protocol. We took different models finetuned with $r_{min}\in \{0.9,0.95,1\}$ as the checkpoint for the second finetune.

As described in the lower part of Tab.~\ref{tab:randcrop}, finetuning again on the KITTI dataset improved the validation accuracy for all starting points (compared to their accuracy on the first finetune). Surprisingly, in the second finetune, repeating the best approach (of randomizing using Eq.~\ref{eq:rcrop_size_range} with $([r_{min},r_{max}] = [0.95,1])$) did not provide the best result. The best approach was to finetune for the second time from a model with a larger range $([r_{min},r_{max}] = [0.9,1])$, thus stronger regularization, but lower EPE in the first finetune. We propose to consider this as additional evidence for the notion that gradually reducing regularization in optical-flow training, helps to achieve a better final local minima.

\noindent \textbf{Full training insights\quad} Concluding Sec.~\ref{experiments:full_train} experiments, we suggest the following: (i) larger scopes can improve optical flow training {\color{black}as long as the regularization provided by small crops is not needed}, {\color{black} (ii) range based crop size randomization (Eq.\ref{eq:rcrop_size_range}) is a good strategy when regularization is needed, }(iii) the training protocol requires strong regularization on early stages, that should be relaxed when possible and (iv) gains on {\color{black}early stages} do not always improve the finetuning accuracy.

%% Experiments - Results

\subsection{Occlusion estimation} 
We evaluated the occlusion estimation of our trained models, using the F1 score, during all stages of the full training. As demonstrated in Tab.~\ref{tab:sintel_finetune_reg}, it appears that gains in optical flow estimation are highly correlated with improvements in occlusion estimation. This might be due to the need for a network to identify non-matchable pixels and to {\color{black} infer} the flow from the context.  Tab.~\ref{tab:occlusion_results} shows a comparison of our F1 score to other reported results, on the full Sintel dataset. Our updated training protocol improves the best reported occlusion result by more than $5\%$.

\subsection{Official Results}
\label{experiments:results}
Evaluating our best models on the MPI Sintel and KITTI benchmarks shows a clear improvement over the IRR-PWC baseline, and an advantage over all other PWC-Net variants. 

\noindent \textbf{MPI Sintel\quad}
We uploaded results for three different versions: (i) with reduced regularization, (ii) with improved zooming schedule and (iii) with the best dynamic scoping approach. As Tab.~\ref{tab:results_sintel_kitti} shows, there is a consistent improvements on the test set. This is congruent with the results in Tab.~\ref{tab:ablation}, obtained on the validation set.


At the time of submission, our method ranks first place on the MPI Sintel benchmark, improving two-frame methods by more than 10\%, surpassing other competitive methods trained on multiple datasets, with multiple frames and all other PWCNet variants, using an equal or larger size of trainable parameters. On the clean pass, we improve the IRR-PWC result by 20 ranks and 7\%. Interestingly, analyzing Sintel categories in Tab.~\ref{tab:results_sintel_kitti}, our model is leading in the categories of fast pixels ($S40_{+}$) and non-occluded pixels, while also producing the best estimation for occluded pixels among two frame methods. This is consistent with our insights on these challenging categories from Sec.\ref{method:scene_scoping}. Fig.~\ref{fig:occ-fast-improve} shows a comparison of our method in the category of fast pixels, with the other two leading methods on Sintel.

\noindent \textbf{KITTI\quad}On KITTI 2012 and KITTI 2015, we saw a consistent improvement of more than
% 12\% and 14.5\%
19.7\% and 12\%, respectively, from the baseline model results, surpassing all other published methods of the popular PWC-Net architecture, and achieving state-of-the art EPE results among two frame methods. Since our training protocol can be readily applied to other methods, we plan, as future work, to test it on other leading architectures.

%% Conclusions
\section{Conclusions}
\label{conclusions}

While a lot of effort is dedicated for finding effective network architectures, much less attention is provided to the training protocol. However, when performing complex multi-phase training, there are many choices to be made, and it is important to understand, for example, the proper way to schedule the multiple forms of network regularization. In addition, the method used for sampling as part of the augmentation process can bias the training protocol toward specific types of samples.

In this work, we show that the conventional scope sampling method leads to the neglect of many challenging samples, which hurts performance. {\color{black}We advocate for the use of larger scopes (crops and zoom-out) when possible, and carefully sample the position of the crop when needed.} We further show how regularization and augmentation should be relaxed as training progresses. The new protocol developed has a dramatic effect on the performance of our trained models and leads to state of the art results in a very competitive domain.

% {\color{blue} I THINK WE SHOULD PRIORITIZE THE SCOPING MESSAGES OVER THE REGULARIZATION ONES AS THEY HAVE MORE NOVELTY AND PRACTICAL IMPLICATIONS
% }

% While pixels with large displacement require large crops in order to stay in the scene (not becoming occluded due to out of bound placement), we show that they also affected by the underlying probability to sample (\ie scope size matters).
% Our approach can be easily tested with other architectures in optical flow or other data-driven domains using fixed sized crops, where there is a spatial meaning for different categories of pixels.
% \fi



%% ---------------  Tables --------------- %%

%%% Experiments

%% Ablation results


% %% Best performance when finetuning sintel comb -> final
% \begin{table}[]
%     \centering
%     \begin{tabular}{@{}l@{~}c@{~}c@{~}c@{~}c@{~}c@{}}
%     \toprule
%     {\begin{tabular}[c]{@{}l@{}}Sintel\\ Model\end{tabular}} & {Dataset} & {\begin{tabular}[c]{@{}c@{}}WD+\\ RN\end{tabular}} & {\begin{tabular}[c]{@{}c@{}}Start\\ From\end{tabular}} & {Epochs} & {\begin{tabular}[c]{@{}c@{}}Val\\ MEPE\end{tabular}} \\ \midrule
%     T3\_SC1 & Sintel comb & v & T3 & 160-450 & 2.119 \\
%     T3\_SC1\_SF & Sintel final & x & T3\_SC1 & 450-790 & \textbf{2.044} \\
%     T3\_SF & Sintel final & x & T3 & 160-450 & 2.149 \\ \bottomrule
%     \end{tabular}
%     \caption{Best performance when finetuning sintel comb -\textgreater final. Zoom in reduced in T3\_SC1\_SF from 1.5 to 1.3.}
%     \label{tab:sintel_finetune_order}
% \end{table}

%% References
\section*{Acknowledgement}
This project has received funding from the European Research Council (ERC) under the European Unions Horizon 2020 research and innovation programme (grant ERC CoG 725974).

==> tables/tables.tex <==
% Occlusions
\newcommand*\TableOcclusions{%
    \begin{table}[]
    \centering
    % \multicols*
    \scalebox{1}{
    \small
    \begin{tabularx}{\linewidth}
    {@{}l@{\hspace{5pt}}X@{}X@{}X@{}c@{}}
    
    %% TABLE COMES HERE
    \toprule
    Method & Clean & Final & Mean & Type \\
    \hline
    \midrule
    FlowNet2~\cite{IMSKDB17} & 0.377 & 0.348 & 0.362 & fwd-bwd \\
    MirrorFlow & 0.39 & 0.348 & 0.369 & CNN \\
    S2DFlow & 0.47 & 0.403 & 0.436 & CNN \\
    ContinualFlow~\cite{Neoral2018ACCV} & - & - & 0.48 & CNN \\
    SelFlow~\cite{Liu:2019:SelFlow} & 0.59 & 0.52 & 0.555 & fwd-bwd \\
    FlowDispOccBoundary~\cite{ISKB18} & 0.703 & 0.654 & 0.678 & CNN \\
    IRR-PWC~\cite{Hur2019CVPR} & 0.712 & 0.669 & 0.690 & CNN \\
    ScopeFlow (Ours) & \textbf{0.740} & {\textbf{0.711}} & \textbf{0.725} & CNN \\ \bottomrule
    \\
    %%
    \end{tabularx}
    }
    \caption{\textbf{Occlusion estimation comparison on Sintel.} All results calculated with F1 measure (higher is better).}
    \end{table}
}

% Ablation
\newcommand*\TableAblation{%
\begin{table*}[ht]
    % \centering
    % \multicols*
    % \setlength{\tabcolsep}{4pt} %% default is 6pt
    \resizebox{\textwidth}{!}{
    \small
    
    
    \begin{tabularx}{\textwidth}
    {@{}c@{\hskip 2pt}|@{\hskip 2pt}c@{\hskip 2pt}|@{\hskip 2pt}c@{\hskip 2pt}|@{\hskip 2pt}@{\hskip 2pt}c@{\hskip 2pt}|c@{\hskip 2pt}|c@{\hskip 2pt}|c@{\hskip 6pt}c@{\hskip 6pt}c@{\hskip 12pt}|c@{\hskip 12pt}c@{\hskip 2pt}|c@{\hskip 2pt}|c@{}}
    \toprule
    Strict OOB & No noise & No decay & Zoom out & Maxcrop & Randcrop & \multicolumn{3}{|c|}{Sintel} & \multicolumn{2}{|c|}{KITTI combined} & Kitti 2012 & Kitti 2015
    \\ \midrule
     &  &  &  &  &  & Train & Val & Test & Train & Val & Test (nooc) & Test (fl-all) \\ \midrule
     \hline
     &  &  &  &  &  & (2.66) & - & 4.57 & (1.33) & - & 3.21 & 7.65 \\ \midrule
    \color{green}\checkmark &  &  &  &  &  & (2.65) & 3.31 & 4.50 & (1.28) & 1.65 & - & - \\ \midrule
    \color{green}\checkmark & \color{green}\checkmark &  &  &  &  & (2.51) & - & - & (1.26) & 1.64 & - & - \\ \midrule
    \color{green}\checkmark & \color{green}\checkmark & \color{green}\checkmark &  &  &  & (2.44) & 3.22 & - & (1.29) & - & - & - \\ \midrule
    \color{green}\checkmark & \color{green}\checkmark & \color{green}\checkmark & \color{green}\checkmark &  &  & - & 3.10 & 4.31 & - & 1.60 & - & - \\ \midrule
    \color{green}\checkmark & \color{green}\checkmark & \color{green}\checkmark &  & \color{green}\checkmark &  & - & 3.00 & - & (1.20) & 1.59 & - & - \\ \midrule
    \color{green}\checkmark & \color{green}\checkmark & \color{green}\checkmark &  &  & \color{green}\checkmark & - & - & - & (1.11) & 1.40 & - & - \\ \midrule
    \color{green}\checkmark & \color{green}\checkmark & \color{green}\checkmark & \color{green}\checkmark & \color{green}\checkmark &  & (2.13) & 2.98 & 4.09 & (1.16)  &	1.59 & - & - \\ \midrule
    \color{green}\checkmark & \color{green}\checkmark & \color{green}\checkmark & \color{green}\checkmark &  & \color{green}\checkmark & - & 2.97 & - & (1.17) & 1.46 & 2.8 & 6.82 \\ \bottomrule
    \\
    \end{tabularx}
    }
    
    \label{tab:ablation}
    \caption{\textbf{Ablation results for our fine tuning experiments.} All results calculated with Mean EPE, except KITTI test results (in progress).}
    \end{table*}
}

% Cropping
\newcommand*\TableCropping{%
    \begin{table}[t]
    \centering
    % \small
    % \resizebox{\linewidth}{!}{
    \begin{tabularx}{0.9\linewidth}
    % {@{}lccccc@{}}
    {@{}lXX@}
    
    \toprule
    Crop size domain / \% per axis
    % & min\_range & max\_range 
    & MEPE & Outliers \\ \midrule %& Pre training \\ \midrule
    \hline
    \multicolumn{1}{l}{Fixed {[}86.4\%, 87.5\%{]}} 
    % & - & - 
    & 1.651 & 0.057 \\
    % & Chairs -\textgreater Things \\ %\midrule
    \multicolumn{1}{l}{Maximal valid crop} 
    % & 100 & 100 
        & 1.594 & 0.059 \\
    % & Chairs -\textgreater Things \\ %\midrule
    \multicolumn{1}{l}{75\%-90\% } 
    % & 75 & 90 
    & 1.472 & 0.052 \\
    % & Chairs -\textgreater Things \\ %\midrule
    \multicolumn{1}{l}{Fixed set {[}(a,b),(c,d),(e,f){]}} 
    % & - & - 
    & 1.466 & 0.053\\ % & Chairs -\textgreater Things \\ %\midrule
    % \multicolumn{1}{l}{50\%-100\% } 
    % % & 50 & 100 
    % & 1.454 & 0.052\\ % & Chairs -\textgreater Things \\ %\midrule
    % \multicolumn{1}{l}{60\%-100\%} 
    % % & 60 & 100 
    % & 1.457 & 0.053\\ % & Chairs -\textgreater Things \\ %\midrule
    % \multicolumn{1}{l}{70\%-100\%} 
    % % & 70 & 100 
    % & 1.455 & 0.053\\ % & Chairs -\textgreater Things \\ %\midrule
    % \multicolumn{1}{l}{75\%-100\%} 
    % % & 75 & 100 
    % & 1.437 & 0.051\\ % & Chairs -\textgreater Things \\ %\midrule
    % \multicolumn{1}{l}{80\%-100\%} 
    % % & 80 & 100 
    % & 1.442 & 0.052\\ % & Chairs -\textgreater Things \\ %\midrule
    % \multicolumn{1}{l}{90\%-100\%} 
    % % & 90 & 100 
    % & 1.435 & 0.053\\ % & Chairs -\textgreater Things \\ %\midrule
    \multicolumn{1}{l}{95\%-100\%} 
    % & 95 & 100 
    & 1.402 & 0.051\\ % & Chairs -\textgreater Things \\
    % %\midrule
    % \multicolumn{1}{l}{97.5\%-100\%} 
    % % & 97 & 100 
    % & 1.455 & 0.053\\ % & Chairs -\textgreater Things \\
    % %\midrule
    \multicolumn{1}{l}{90\%-100\% -\textgreater 95\%-100\%} 
    % & 95 & 100 
    & \textbf{1.377} & \textbf{0.051} \\ %& 90\%-100\% model \\
    %\midrule
    \multicolumn{1}{l}{max crop -\textgreater 95\%-100\%} 
    % & 95 & 100 
    &  &  \\ %& Max crop model \\ %\midrule
    \multicolumn{1}{l}{95\%-100\% -\textgreater 95\%-100\%} 
    % & 95 & 100
    &  &  \\ %& 95-100 model \\
    % \midrule
    \bottomrule
    \\
    \end{tabularx}
    % }
    \label{tab:randcrop}
    \caption{\textbf{Comparison of cropping approaches.} MEPE and outlier percentage ($>3$ px) on KITTI combined validation (in progress).}
    
    
    \end{table}
}


% Sintel, KITTI ALL
\newcommand*\TableSintelKITTI{%
    \begin{table*}[t]
    \centering
    \tiny
    \resizebox{\textwidth}{!}{
    \begin{tabularx}{\textwidth}
    % {@{}lcccccccccccc@{}}
    {@{}l@{}|X@{}X@{}X@{}X@{}X@{}X@{}X@{}|X@{}|X@{}X@{}|X@{}|X@{}}
    \toprule
    
    \multirow{3}{*}{\textbf{Method}} & \multicolumn{8}{|c|}{\textbf{Sintel}} & \multicolumn{3}{|c|}{\textbf{KITTI}} & \multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}MEPE & \\ ALL\end{tabular}}} \\ \cmidrule(lr){2-12}
     & \multicolumn{7}c{\textbf{Final pass}} & \multicolumn{1}{|c|}{\textbf{Clean pass}} & \multicolumn{2}{c}{\textbf{2012}} & \multicolumn{1}{|c|}{\textbf{2015}} &  \\
     & \multicolumn{1}{c}{all} & \multicolumn{1}{c}{matched} & \multicolumn{1}{l}{unmatched} & \multicolumn{1}{c}{d0-10} & \multicolumn{1}{l}{d60-140} & \multicolumn{1}{c}{s0-10} & \multicolumn{1}{l}{s40+} & \multicolumn{1}{c}{all} & \multicolumn{1}{c}{Out-All} & \multicolumn{1}{c}{Avg-All} & \multicolumn{1}{c}{Fl-all} &  \\ \midrule
    FlowNet2 \cite{IMSKDB17} & 5.739 & 2.752 & 30.108 & 4.818 & 1.735 & 0.959 & 35.538 & 3.959 & 8.8 & 1.8 & 10.41 & 3.833 \\
    InterpoNet\_ff\cite{Zweig_2017_CVPR} & 5.535 & 2.372 & 31.296 & 4.72 & 1.532 & 1.064 & 32.633 & 3.952 & 14.76 & 2.6 & 22 & 4.029 \\
    LiteFlowNet\cite{hui18liteflownet} & 5.381 & 2.419 & 29.535 & 4.09 & 1.729 & 2.747 & 34.722 & 4.539 & 7.27 & 1.6 & 9.38 & 3.840 \\
    MR-Flow\cite{Wulff:CVPR:2017} & 5.376 & 2.818 & 26.235 & 5.109 & 1.755 & 0.908 & 32.221 & 2.527 & - & - & 12.19 & - \\
    DCFlow\cite{xu_2017_dcflow} & 5.119 & 2.283 & 28.228 & 4.665 & 1.44 & 1.052 & 29.351 & 3.537 & - & - & 14.86 & - \\
    PWC-Net\cite{Sun2018PWC-Net}* & 5.042 & 2.445 & 26.221 & 4.636 & 1.475 & 2.986 & 31.07 & 4.386 & 8.1 & 1.7 & 9.6 & 3.709 \\
    ProFlow\cite{Maurer2018ProFlowLT} & 5.017 & 2.596 & 24.736 & 5.016 & 1.601 & 0.91 & 30.715 & 2.709 & 7.88 & 2.1 & 15.04 & 3.275 \\
    LiteFlowNet2\cite{hui19liteflownet2} & 4.903 & 2.346 & 25.769 & 4.142 & 1.546 & 0.797 & 31.039 & 3.187 & 6.16 & 1.4 & 7.62 & 3.163 \\
    PWC-Net+\cite{Sun2018:Model:Training:Flow}*+ & 4.596 & 2.254 & 23.696 & 4.781 & 1.234 & 2.978 & 26.62 & 3.454 & 6.72 & 1.4 & 7.72 & 3.150 \\
    HD3-Flow\cite{yin2019hd3} & 4.666 & 2.174 & 24.994 & 3.786 & 1.647 & 0.657 & 30.579 & 4.788 & 5.41 & 1.4 & 6.55 & 3.618 \\
    IRR-PWC\cite{Hur2019CVPR}*\textasciicircum{} & 4.579 & 2.154 & 24.355 & 4.165 & 1.292 & 0.709 & 28.998 & 3.844 & 6.7 & 1.6 & 7.65 & 3.341 \\
    MFF\cite{ren2018fusion}*+ & 4.566 & 2.216 & 23.732 & 4.664 & 1.222 & 0.893 & 26.81 & 3.423 & 7.87 & 1.7 & 7.17 & 3.230 \\
    ContinualFlow\_ROB\cite{Neoral2018ACCV}*+ & 4.528 & 2.723 & 19.248 & 5.05 & 1.713 & 0.872 & 26.063 & 3.341 & - & - & 10.03 & 3.935 \\
    VCN\cite{yang2019vcn} & 4.52 & 2.195 & 23.478 & 4.423 & 1.357 & 0.934 & 26.434 & 2.891 & - & - & 6.3 & - \\
    SelFlow\cite{Liu:2019:SelFlow}* & 4.262 & 2.04 & 22.369 & 4.083 & 1.287 & 0.582 & 27.154 & 3.745 & 6.19 & 1.5 & 8.42 & 3.169 \\
    ScopeFlow*, no scoping changes & 4.503 & 2.16 & 23.607 & 4.124 & 1.292 & 0.706 & 27.831 & 3.86 & - & - & - & - \\
    ScopeFlow*, no cropping changes & 4.317 & 2.086 & 22.511 & 4.018 & 1.311 & 0.739 & 26.218 & 3.696 & - & - & - & - \\
    ScopeFlow* (Ours) & 4.098 & 1.999 & 21.214 & 4.028 & 1.18 & 0.725 & 24.477 & 3.592 & 5.96 & 1.4 & 6.82 & \textbf{3.030} \\ \bottomrule
    \\
    \end{tabularx}
    }
    \caption{\textbf{Public benchmarks results comparison.} Models with comparable architecture (PWC-Net) are marked with *, Models using extra data in finetune marked with +, Our baseline model marked with \textasciicircum{}, We get the best EPE results in both Sintel and KITTI2012 benchmarks, surpassing all other comparable variants of our baseline model on KITTI2015, with a considerable improvement to our baseline. All scores were taken on the day of upload.}
    \label{tab:results_sintel_kitti}
    \end{table*}
}

% Sintel finetune improvements applied on FlyingChairs
\newcommand*\TableFChairs{%
\begin{table*}[]
\begin{tabular}{llllllll}
\hline
\multicolumn{1}{c}{\textbf{FlyingChairs model}} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Random\\ zooming\\ ranges\end{tabular}}} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Weight decay\\ +\\ Random noise\end{tabular}}} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}FChairs \\ val\\ MEPE\end{tabular}}} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Sintel comb\\ MEPE\end{tabular}}} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Val\\ MEPE\end{tabular}}} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Sintel comb\\ MEPE\end{tabular}}} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Sintel comb\\ OCC F1\end{tabular}}} \\ \hline
ChairsAuthors & 1;1.5 & v & - & 3.138 & 1.8433 & \textbf{2.613} & 0.662 \\
ChairsNRegZout & 0.8,1.5 & x & 1.622 & 3.264 & 1.8292 & 2.544 & 0.665 \\
ChairsNRegZoutRZin & 0.8,1.3 & x & 1.597 & 3.321 & \textbf{1.8172} & 2.545 & \textbf{0.666} \\ \hline
\end{tabular}
\caption{Regularization is needed in early stages. Dont reduce aug (zoom in) during pre-training. All trained from initialized weights for 108 epochs}
\label{tab:chairs_training}
\end{table}
}

% Sintel finetune improvements applied on FlyingThings
\newcommand*\TableFThingsBS{%
\begin{table*}[]
\begin{tabular}{llllllll}
\hline
\multicolumn{1}{c}{\textbf{FlyingThings3D model}} & \multicolumn{1}{c}{\textbf{Checkpoint}} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Val\\ MEPE\end{tabular}}} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Sintel comb\\ MEPE\end{tabular}}} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Sintel comb\\ MEPE\end{tabular}}} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Val\\ MEPE\end{tabular}}} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Sintel comb\\ MEPE\end{tabular}}} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Sintel comb\\ OCC F1\end{tabular}}} \\ \hline
CThingsAuthors & Downloaded & - & 2.645 & 3.138 & 1.8433 & \textbf{2.613} & 0.662 \\
CThingsBS6 & ChairsAuthors & 1.876 & 2.639 & 3.264 & 1.8292 & 2.544 & 0.665 \\
CThingsBS2 & ChairsAuthors & 1.843 & 2.613 & 3.321 & \textbf{1.8172} & 2.545 & \textbf{0.666} \\ \hline
\end{tabular}
\caption{Smaller batch size is slightly better in early training. All trained for 50 epochs with the original crop size {[}384,768{]}, weight decay and random noise, and the original zooming range of {[}1,1.5{]}.}
\label{tab:things_training_bs}
\end{table}
}

% FThings regularization and overtraining effect
\newcommand*\TableThingsReg{%
\begin{table*}[]
\begin{tabular}{lllllll}
\hline
\multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}FlyingThings3D \\ model\end{tabular}}} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Random\\ zooming\\ ranges\end{tabular}}} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Weight decay\\ +\\ Random noise\end{tabular}}} & \multicolumn{1}{c}{\textbf{Checkpoint}} & \multicolumn{1}{c}{\textbf{Epochs}} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Val\\ MEPE\end{tabular}}} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Sintel comb\\ MEPE\end{tabular}}} \\ \hline
CThingsBS2 & 1;1.5 & v & CThingsAuthors & 109-159 & 1.843 & \textbf{2.613} \\
CThingsRegMcrop & 0.8,1.5 & v & ChairsNRegZout & 109-159 & 1.829 & 2.544 \\
CThingsNRegMcropOverTrain & 0.8,1.5 & x & CThingsRegMcrop & 159-165 & \textbf{1.817} & 2.545 \\ \hline
\end{tabular}
\caption{FThings regularization and overtraining effect. Gains can come from checkpoints with inital higher MEPE. Don't over train, don't reduce reg, on early stages all get same Occ F1.}
\label{tab:things_training_reg}
\end{table}
}

% Higher gains in early stages doesn't always translate to fine-tune gains
\newcommand*\TablePreTrainEffectKITTI{%

}

% Reduce reg in finetune
\newcommand*\TableRegInFinetuneSintel{%
}

% Best performance when finetuning sintel comb -> final
\newcommand*\TableSintelTrainOrder{%
}
